Time Window Frechet and Metric-Based Edit Distance for Passively Collected Trajectories

The advances of modern localization techniques and the wide spread of mobile devices have provided us great opportunities to collect and mine human mobility trajectories. In this work, we focus on passively collected trajectories, which are sequences of time-stamped locations that mobile entities visit. To analyse such trajectories, a crucial part is a measure of similarity between two trajectories. We propose the time-window Frechet distance, which enforces the maximum temporal separation between points of two trajectories that can be paired in the calculation of the Frechet distance, and the metric-based edit distance which incorporates the underlying metric in the computation of the insertion and deletion costs. Using these measures, we can cluster trajectories to infer group motion patterns. We look at the $k$-gather problem which requires each cluster to have at least $k$ trajectories. We prove that k-gather remains NP-hard under edit distance, metric-based edit distance and Jaccard distance. Finally, we improve over previous results on discrete Frechet distance and show that there is no strongly sub-quadratic time with approximation factor less than $1.61$ in two dimensional setting unless SETH fails.

==> intro.tex <==
\subsection{Combinatorial Representations of Trajectories}
We consider a combinatorial representation of human motion trajectories. In this formulation, the domain is partitioned into cells (labeled) and a trajectory is represented as a sequance of cells visited in this order, possibly associated with the time window of visit for each cell. This representation is motivated in two ways. First, a variety of trajectory sensing schemes use this formulation explicitly. For example, in the indoor scenario, laser sensors called tripwires can be placed inside the building to detect subject crossing. A typical tripwire sensor can be considered as a pair of wireless transmitter and receiver using highly directional signals (laser, infrared, etc). The transmitter is typically mounted at the boundary of one obstacle and the receiver is placed at another point with line of sight visibility. Any user crossing the tripwire can be detected and the crossing direction can be inferred -- for example, by using a pair of lasers and comparing the time of crossings. Surveillance cameras can also be used for the same purposes. See Figure~\ref{fig:trajectory} for an example.

In the scenario of vehicle tracking, vehicles only travel on a predefined road map. It is a common practice to decompose the road map into road segments. Each segment is bounded between two adjacent intersections. GPS trajectories are often mapped to the road network and can be easily turned into a sequence of road segments visited in this order.  Taking the combinatorial representation can possibly save tremendously in terms of storage without losing much information, especially in the case of the road segment, as many GPS samples can be taken when the vehicle travels on the same road segments. 

%\begin{figure}[htpb]
%	\centering
%	\includegraphics[width=0.75in]{trajectory}
%	\caption{A trajectory traced out by tripwire sensors, represented as a sequence of cells visited $1, 2, 3, 4, 5, 2$.}
%	\label{fig:trajectory}
%\end{figure}

Generally speaking, one can use the representation as either the sequence of tripwire sensors crossed (with direction of crossing), or the sequence of the cells visited, in which the cells are the faces of the planar decomposition by the tripwire sensors or in the road segment decomposition of the road map. These two representations are equivalent if every tripwire sensor separates two cells (or, each cell is simply connected). In the following we use the sequence of cells and denote this as the \emph{string representation} of a trajectory with respect to a planar decomposition $\Sigma$. 

In the following we may use both the \emph{time-stamped} string representation, in which each cell appearance in the trajectory is associated with a time window, or the non-timestamped version, without the time information. The latter can be interesting when either the temporal information is unavailable, or when the geometric \emph{shape} of the trajectory is of main interest. The choice of the representation can be determined by the type of structures that the applications wish to preserve. In the following we discuss this aspect and show a variety of popular trajectory mining tasks. 

==> jaccardHard.tex <==
\subsection{Hardness on the Jaccard Distance}
\label{sec:hardnessJacc}
%\subsection{Jaccard Distance}
A trajectory with string representation can be processed as a set of \emph{$w$-shingles}. 
%A $w$-shingle is a continuous sequence of $w$ items from a given sequence, which is widely used in processing text and speech in natural language processing. 
%In our setting, 
\begin{definition}[$w$-shingle]
A $w$-shingle is a sequence of $w$ consecutive location strings on trajectory with string representation.
\end{definition}
We combine all $w$-shingles from each trajectory into a set. 
Thereafter, we introduce Jaccard distance over the set of $w$-shingles as a metric between two trajectories. 
\begin{definition}[Jaccard distance]
For two sets $A$ and $B$,
the \emph{Jaccard distance} is defined as $$d(A,B) = 1-\frac{\left | A \cap B \right |}{\left | A \cup B \right |}.$$

\end{definition}

Computing the Jaccard distance between two trajectories with $O(n)$ locations  can be done in $O(nw)$ time. 

\begin{theorem}
	The $k$-gather problem on trajectories with Jaccard distance is NP-hard. 
\end{theorem}
\begin{proof}
	The proof use the same gadget as Theorem \ref{theo:edit}. 
There is a solution to the $k$-gather problem if and only if the maximum radius of clusters with Jaccard distance on $2-$shingles is $\frac{15}{8n+10}$. 
%with a cluster radius of $\frac{5}{4n+7}$ with respect to the Jaccard distance metric on the set of $2$-shingles of the trajectories. 
%	The minimum Jaccard distance from the center  trajectory of a cluster to the  trajectories in other cluster is $\frac{7}{4n+9}$.  Therefore, it has approximation hardness of $1.4$.

\end{proof}





\subsection{Approximation Algorithm}
\label{sec:approxAlgo}

Fortunately for the $k$-gather problem there is a $2$-approximation algorithm as proved in \cite{aggarwal2006achieving}. 
We provide an approximation algorithm to find out the minimum radius for $k$-gather problem with the above distance metrics.
First, we compute the distance for all pairs of trajectory strings.
We try all the values of distance to be the radius $R$ of the $k$-gather clustering, so that  we find the smallest $R$ satisfying the two conditions:
\begin{enumerate}
  \item  There are at least $k-1$ other points within  the distance of $R$ taking each point as the center. 
  \item Initially mark all the points as uncovered , let the set of center of cluster $C$ be an empty set.Denote the set of points representing trajectories as $V$. 
    Repeat the following procedure until all points are covered: select an arbitrary unmarked point $v\in V$ as a center. If there is any uncovered point within the distance of $R$ from $v$,  we add $v$ to $C$, and mark all the  points within distance $R$ from $v$ as covered.
   
    Thereafter, we create a flow network as following. Create a source $s$,  sink $t$, nodes for each center in $C$ and nodes for each vertex in $V$. For each center $c\in C$, add edges from $s$ to $c$  with capacity $k$; meanwhile add edges with unit capacity from $c$ to all the points that are within distance $R$ from $c$ .
    For each point $v \in V$, add edges from $v$ to $t$ with unit capacity.
    Check if there is a flow of capacity $k\left | C \right |$ from $s$ to $t$. 
    If so, the flow provides a solution for $k$-gather. If not, exit with failure.
    
    
\end{enumerate}
